DICE: Dynamic Interconnections for the Cellular Ecosystem

To enable roaming of users, the cellular ecosystem integrates many entities and procedures, including specific infrastructure to connect Mobile Network Operators (MNOs), business partnerships or the use of third-party Data Clearing Houses (DCHs) for billing. Many of these rely on specifications rooted in dated and arcane practices, involving long waiting periods for financial clearing, complex billing models, and disparate mechanisms for dealing with inter-MNO disputes. In this paper, we propose a novel solution, DICE (Dynamic Interconnections for the Cellular Ecosystem), aimed at facilitating dynamic collaboration between MNOs, and sustain fluid interconnection models between the end-users and MNOs. DICE uses distributed ledger technology (DLT) to enable MNOs to interact directly, and offer customizable services to their users through the use of crypto-currencies. We leverage real-world data from a major operational MNO in Europe to support our claims, and to extract the requirements for the DICE system. We introduce the DICE protocol, and discuss real-world implementation considerations.

==> sections/background.tex <==
% !TeX root = paper.tex
% ================================================================


\subsection{Roaming Overview}

Roaming is one of the fundamental features of the cellular networks ecosystem. 
It enables clients of one \ac{MNO} to use the network of another \ac{MNO} 
when traveling outside their provider's area of coverage, nationally or 
internationally.

To support roaming, both \acp{MNO} must have a functioning technical solution 
and a commercial agreement in place. MNOs negotiate agreements, implement and test 
the roaming technical solution of choice and enable interworking. Interworking is 
defined as the entirety of technical, commercial and operational means necessary to 
join the service platforms of two \acp{MNO}, including all parties in the chain, 
to enable a minimum of two end users to use a specific service offered by both 
\acp{MNO} across their network boundaries. With the technical solution in place, 
commercial roaming can be enabled and MNOs' customers can use their respective 
partners' networks to extend coverage. Figure~\ref{fig:roaming_flow} shows a simple 
process-flow diagram with an overview of these steps.

\begin{figure}[t] 
	\centering
		\includegraphics[width=.98\columnwidth]{fig/Roaming_flow_process.pdf}%
    \vspace{-3mm}
	\caption{\small Flow diagram for roaming establishment process.} 
	\vspace{-5mm}
	\label{fig:roaming_flow}
\end{figure}

Once a commercial agreement has been established, 
a number of technical roaming testing are carrying on including testing and coordination over 
the signaling platform and testing the \ac{IPX} connectivity. Signaling is a prerequisite to 
testing, as it is the basis for the communication between the two networks. The \ac{IPX} is 
a centralized IP network that provides routing, interconnection and additional services for 
MNOs GPRS traffic. It is a secure and private inter-operator packet data network that allows 
MNOs to extend their coverage world-wide. 

Companies are increasingly recognizing the value of roaming to their business, 
no longer seeing it simply as an implementation and management function. 
Thus, companies are splitting the work between operational Roaming and commercial Roaming.
  
Once all roaming testing is completed and interworking established, commercial roaming starts and MNOs can 
recover roaming revenues. 
%After all roaming testing is completed and interworking established, MNOs must test the 
%billing function key to recovering roaming revenue. 
To recover roaming revenue, \acp{MNO}  
must exchange billing information on an agreed-upon format of the \ac{TAP} files, following 
the recommendations offered by the \ac{GSMA}. These files record the activity of roaming clients 
in a specific \ac{VMNO} and enable the \ac{VMNO} to claim revenue from the partner \ac{HMNO} for 
this client. Although it is possible to do this on a peer-to-peer basis, most \acp{MNO} choose to 
exchange \ac{TAP} files via \acp{DCH}. DCHs can provide a single point of contact to send and 
distribute these files between roaming partners, they also provide other functions, 
including \ac{TAP} file creation and validation, fraud detection, \ac{IOT} verification and re-rating,
and may serve as Financial Clearing Agent (FCH), producing, exchanging and clearing 
invoices. 


%*******************************************************************************
\subsection{Roaming Solutions}

% Other options include multi-IMSI solutions or Network Extensions.
In terms of business agreement solutions, the most popular option for \acp{MNO} is the 
standard bilateral agreement. Over the last years, bilateral roaming is reaching its limits, 
impacting on current coverage requirements for voice and data quality of service and the 
introduction of new services such as \acp{VoLTE}. New bilateral roaming agreements for 
roaming and interworking are costly and are generally of lower value today. Even more, 
smaller and newer operators have great difficulty entering this market and extending their 
international coverage even for basic voice services. 

The challenges for the bilateral roaming model have motivated a new model that relies on 
the roaming hubbing solution. In this model, operators connect to a hubbing 
solution provider to gain access to many roaming partners, externalizing the interworking 
establishment to the roaming hub provider. 
Hubs are then interconnected to further expand potential operator relationships.  
The roaming hubbing solution does not preclude the existence of bilateral agreements between 
\acp{MNO} and can be viewed as a complement to the bilateral roaming model.

The Roaming Hub must offer a set of mandatory services, including agreement management, 
signaling, testing, operations and maintenance (troubleshooting). It may also support a set of 
complimentary services, such as data clearing (i.e., acting as a DCH), fraud 
prevention, financial clearing, global roaming quality guarantees or financial liability. 

To support LTE roaming, \acp{MNO} commonly connect with each other through an \ac{IPX} network. 
An \ac{IPX}~\cite{ipx-gsm-whitepaper, ipx-gsm-guidelines} can be described as a private IP 
backbone network that interconnects \acp{MNO} and may be run by a third party (IPX provider).  
An IPX provider has connections to multiple network operators and thus enables each MNO to 
connect to other operators via a single point of contact, thus offering the Roaming Hub 
function (and the services that this provides). 

\begin{figure}[t] 
	\centering
		\includegraphics[width=.98\columnwidth]{fig/roaming_IPX_solutions.pdf}%
    \vspace{-3mm}
	\caption{\small IPX Architecture and network configurations for roaming.} 
	\vspace{-5mm}
	\label{fig:roaming}
\end{figure}

When a commercial agreement exists between two \acp{MNO}, there are multiple network 
configurations to enable roaming between the two networks. Figure~\ref{fig:roaming} presents 
a set of architecture configurations that can be used for roaming in a mobile network -- 
\ac{HR}, \ac{LBO} and \ac{IHBO}.

When a mobile node is at home (Figure~\ref{fig:roaming}, left), the \textit{home user}'s traffic will take 
a short path inside the network to reach a suitable \ac{PGW} to the Internet. 
The traffic of a \textit{roaming user} (Figure~\ref{fig:roaming}, right) is directed to an egress \ac{PGW} 
whose location depends on the roaming architecture.  
In the case of \ac{HR}, the mobile node receives the IP address from its home \ac{MNO} and the 
\textit{roaming user}'s traffic is first routed towards a \ac{PGW} in the \textit{home network} 
(red path).
With \ac{LBO}, the mobile node receives its IP address from the visited network and the traffic is 
routed towards a local \ac{PGW} in the \textit{visited network} (purple path). 
When using \ac{IHBO}, the mobile node obtains its IP address from the IPX networks and the traffic 
is routed through a \ac{PGW} in the \ac{IPX} network (green path).
This strikes a middle ground as the \ac{PGW} may be chosen close to the visited network to minimize 
overhead and, at the same time, the IP address may be assigned in a way that it is recognized by the 
home network so that the roaming user can access local services.

The particular roaming configuration topology can have a potential impact on the communication performance. 
For instance, when the node accesses services inside the \textit{visited network}, the performance may be
worse in the \ac{HR} case, because all packets travel twice between the visited and the home 
network. Previous work has found that the default roaming configuration currently used in majority of MNOs in 
Europe is the home routed roaming~\cite{mandalari2018experience}.

\subsection{Related Work}


==> sections/mechanism.tex <==
% !TeX root = paper.tex
% ================================================================


\subsection{DICE Protocol}
The actors that interact in DICE are the following: 
\begin{itemize}
\item Mobile Node (i.e., the roamer or the end user roaming in a foreign country), 
\item HPMN: the home public mobile networks), 
\item VPMN: the visited public mobile network), 
\item HHub: the the home network roaming hub and 
\item VHub: the visited network roaming hub (this can be the same as the HHub). 
\ael{include here a schema of the interactions and the different steps we define}
\end{itemize}

To become part of DICE, each MNO must first initialize a DICE peering node and connect to the distributed ledger. 
Each MNO publishes (\ael{off-chain?}) the technical data related to international roaming and interworking, tariff and contact information for roaming partners. 
This also integrates information about the agreements between the MNOs and Roaming Hub providers (IPX service). 
Currently, GSMA offers this type of service through the Roaming Agreement EXchange (RAEX) initiative, which more than 500 MNOs are now using. 
\ael{should we still rely on GSMA for managing this type of service?}

The MN signs a service contract with the HPMN, and receives an e-wallet for roaming services.
The HPMN generates roaming coins and transfers to the Mobile Node (MN) a quantity agreed as part of their contract. 
When the MN is roaming in the visited country, it receives service offers from the local operators. 
The HPMN has special roaming agreements with the VPMN that translate into lower costs and advantageous offers for the MN.  
The MN selects a VPMN and configures its eSIM with a new profile to become a native customer of the VPMN. 
\ael{I guess here we need a legal framework in order to enable the MN to become a customer of the VPMN. The HPMN should also sign this "roaming service" contract.}

The communication transactions between the VPMN and the MN will generate a bill which the MN pays to VPMN with coins. 
The MN is the actor in charge to verify that it gets the service that the VPMN proposed.
The VPMN can then use these coins to claim the actual payment from the HPMN.

The consortium uses the DL to store coin transactions (i.e., who owns which coins). 
The consensus mechanism does not takes into account the amount of traffic exchanged, it track exclusively the amount of roaming coins transferred.

I guess the IPX can also be paid out of these coins (especially in the case of the IPX connecting the VMNO. 
The VMNO can use some of these coins to pay to IPX for the traffic generated by the specific MN who paid the coins.


\subsection{DICE Billing Approach}

\paragraph{Option 1: } Suppose now a very simple model where 1 roaming coin = 1 MB of data = 1 euro.
%It is the MN who verifies that it gets what it pays for .
So, the MN pays 1 coin and it verifies that he has sent 1 MB of data.  It does not pay another coin while it still has not completed the 1 MB of data sent.
\ael{is the latter point feasible though? Wouldn't this results in a very high number of transactions in the ledger?}

The billing system depends on a service in the MN. The HMNO must install this piece of software in the MN operating system. If this is part of a 3GPPP standard, than this is a proper function and it should be expected to be there. The main question is whether this trust model is acceptable or not. I guess it is a middle ground between Home routing and LBO. In home routing, the HMNO verifies all the traffic, so it doesnt have to trust anyone (well, it needs to trust the DCH, in case of divergence with the VMNO data). In LBO, the HMNO needs to fully trust the VMNO, which i guess they dont trust. In this solution, there is agent in the MN that verifies the traffic consumed. What is the threats here? Clearly, the MN cannot spend less coins than needed, because the VMNO wouldnt give it access any more. The MN can potentially spend more coins than needed. Why would it do that? I guess the problem here is if the VMNO somehow hacks the MN and gets it transfer the coins without using the data quota (you could think that the MN and VMNO can collude and cash the coins from the HMNO and split the gains, not sure if this makes a lot sense.

In this model of 1 coin = 1 euro = 1MB, i guess we can support some billing models and not others.

\paragraph{Option 2: } 
If we remove one of the constraints and we keep 1 coin = 1 MB, then the translation into euros is done when the VMNO wants to cash the coins from the HMNO. Please note that the DL contain information about when each transaction was made, so it is potentially possible to determine the peak of traffic (this needs to be evaluated, especially in the light of off chain transactions, which may turn this much harder).

